InstructPart: Task-Oriented Part Segmentation with Instruction Reasoning

Large multimodal foundation models, particularly in the domains of language and vision, have significantly advanced various tasks, including robotics, autonomous driving, information retrieval, and grounding. However, many of these models perceive objects as indivisible, overlooking the components that constitute them. Understanding these components and their associated affordances provides valuable insights into an object's functionality, which is fundamental for performing a wide range of tasks. In this work, we introduce a novel real-world benchmark, InstructPart, comprising hand-labeled part segmentation annotations and task-oriented instructions to evaluate the performance of current models in understanding and executing part-level tasks within everyday contexts. Through our experiments, we demonstrate that task-oriented part segmentation remains a challenging problem, even for state-of-the-art Vision-Language Models (VLMs). In addition to our benchmark, we introduce a simple baseline that achieves a twofold performance improvement through fine-tuning with our dataset. With our dataset and benchmark, we aim to facilitate research on task-oriented part segmentation and enhance the applicability of VLMs across various domains, including robotics, virtual reality, information retrieval, and other related fields. Project website: https://zifuwan.github.io/InstructPart/.

==> tabels/instruction_referring.tex <==
\begin{table}[htb]
  \renewcommand\arraystretch{1.05}
  \centering
  \footnotesize
  \caption{Instruction referring part segmentation results.}
  \vspace{-3.6mm}
  \centering
     \setlength{\tabcolsep}{1.0mm}{\begin{tabular}{l|cccc|cccc}
      \specialrule{.1em}{.05em}{.05em} 
      \multirow{2}{*}{Methods}& \multicolumn{4}{c|}{Human-annotated} & \multicolumn{4}{c}{GPT-4-rewrote}\\
              & gIoU   & cIoU  & $\text{P}_{\text{50-95}}$   & $\text{P}_\text{50}$  & gIoU   & cIoU  &  $\text{P}_{\text{50-95}}$  & $\text{P}_\text{50}$  \\
        \hline\hline
        VLPart~\cite{sun2023going}   & 0.32 & 0.94 & 0.06 & 0.15 & 0.46 & 0.97 & 0.20 & 0.44 \\
        \hline
        OVSeg~\cite{liang2023open}   & 16.44 & 13.11 & 5.34 & 10.74 & 16.93 & 14.21 & 4.67 & 10.89 \\
        SAN~\cite{xu2023side}  & 9.03 & 13.99 & 2.70 & 6.10 & 9.02 & 15.87 & 2.79 & 6.39 \\
        \hline
        X-Decoder~\cite{zou2023generalized}  & 9.92 & 10.62 & 3.32 & 6.97 & 9.51 & 9.74 & 2.99 & 6.68 \\
        SEEM~\cite{zou2023segment}  & 7.80 & 9.88 & 2.00 & 4.50 & 9.39 & 11.67 & 2.55 & 6.53 \\
        TRIS~\cite{liu2023referring}  & 14.74 & 14.85 & 3.53 & 9.58 & 15.47 & 15.56 & 3.95 & 10.89 \\
        G-SAM~\cite{kirillov2023segment,liu2023grounding}  & 22.11 & 19.79 & 7.16 & 15.67 & 22.38 & 19.60 & 7.30 & 15.53 \\
        \hline
        LISA~\cite{lai2023lisa}  & 26.06 & 28.63 & 14.15 & 23.08 & 26.25 & 30.14 & 13.72 & 24.38 \\
        Shikra-S~\cite{chen2023shikra,kirillov2023segment}  & 2.76 & 4.33 & 1.26 & 2.18 & 8.59 & 11.38 & 4.38 & 6.82 \\
        VisionLLM  & -- & -- & -- & -- & -- & -- & -- & -- \\
        \hline
        SAM-GPT-4V  & -- & -- & -- & -- & -- & -- & -- & -- \\
        \hline
        Average & 12.13 &	12.90 &	4.39 &	8.77 &	13.11 &	14.34 &	4.72 &	9.83 \\
        \specialrule{.1em}{.05em}{.05em} 
\end{tabular}}
\vspace{-3mm}
  \label{tab:instruct_refer}
\end{table}

==> tabels/oracle_referring.tex <==
\begin{table}[]
  \renewcommand\arraystretch{1.05}
  \centering
  \footnotesize
  \caption{Oracle referring part segmentation results.}
  \vspace{-3.6mm}
  \centering
     \setlength{\tabcolsep}{1.0mm}{\begin{tabular}{l|cccc|cccc}
      \specialrule{.1em}{.05em}{.05em} 
      \multirow{2}{*}{Methods}& \multicolumn{4}{c|}{Object-Part} & \multicolumn{4}{c}{Object-Part-Affordance}\\
              & gIoU  & cIoU  & $\text{P}_{\text{50-95}}$   & $\text{P}_\text{50}$  & gIoU   & cIoU  &  $\text{P}_{\text{50-95}}$  & $\text{P}_\text{50}$  \\
        \hline\hline
        VLPart~\cite{sun2023going}   & 15.11 & 17.93 & 11.44 & 15.38 & 13.56 & 12.15 & 10.86 & 13.64 \\
        \hline
        OVSeg~\cite{liang2023open}   & 20.86 & 17.78 & 7.21 & 15.67 & 20.61 & 17.59 & 7.07 & 15.53 \\
        SAN~\cite{xu2023side}  & 13.45 & 19.70 & 5.36 & 10.74 & 14.72 & 20.17 & 5.86 & 12.19 \\
        \hline
        X-Decoder~\cite{zou2023generalized}  & 8.76 & 10.90 & 2.79 & 5.66 & 9.64 & 11.47 & 3.11 & 6.53 \\
        SEEM~\cite{zou2023segment}  & 8.29 & 11.66 & 2.53 & 5.37 & 8.29 & 11.66 & 2.53 & 5.37 \\
        TRIS~\cite{liu2023referring}  & 17.04 & 17.28 & 5.12 & 11.76 & 17.05 & 17.28 & 5.01 & 12.19 \\
        G-SAM~\cite{kirillov2023segment,liu2023grounding}  & 26.21 & 22.47 & 10.09 & 19.30 & 25.71 & 22.43 & 9.78 & 18.87 \\
        \hline
        LISA~\cite{lai2023lisa}  & 35.91 & 41.36 & 20.55 & 34.98 & 36.67 & 42.91 & 20.87 & 35.56 \\
        Shikra-S~\cite{chen2023shikra,kirillov2023segment}  & 37.74 & 33.89 & 24.37 & 36.87 & 35.44 & 32.64 & 21.94 & 33.24 \\
        VisionLLM  & -- & -- & -- & -- & -- & -- & -- & -- \\
        \hline
        SAM-GPT-4V  & -- & -- & -- & -- & -- & -- & -- & -- \\
        \hline
        Average & 20.37 & 21.44 & 9.94 &	17.30 &	20.18 &20.92 &	9.67 &	17.01 \\


        \specialrule{.1em}{.05em}{.05em} 
\end{tabular}}
\vspace{-3mm}
  \label{tab:oracle_refer}
\end{table}

==> tabels/table1.tex <==
\begin{table*}[htbp]
\renewcommand\arraystretch{0.88}
\newcommand{\cc}{\cellcolor{gray!20}}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.2cm}
\begin{center}
\caption{\textbf{Performance comparison with the state-of-the-art SGG methods for the PredCls task on the corrupted Visual Genome \cite{krishna2017visual} dataset}.  We report the accuracy in percentage for the mR@20: UC/C, mR@50: UC/C, mR@100: UC/C metrics, structured in six rows. The best results for each metric are in \textbf{bold}. The last column reports the average mean recall across all 20 types of corruption, and the percentage decrease in \textcolor{MidnightBlue}{blue} when compared to the mean recall on clean images. $^\dag$We evaluate these methods using the codes provided by the authors.}
\label{tab:performance2}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|cccccccccccccccccccc|cc}
\toprule
& Method & gaus & shot & imp & dfcs & gls & mtn & zm & snw & frst & fg & brt & cnt & els & px & jpg & sun & wtd & smk & rain & dust & Average mR \\			
\midrule
\multirow{6}{*}[-0.9ex]{\centering \rotatebox{90}{mR@20: C/UC}}&GB-Net$^\dag$~\cite{zareian2020bridging} & 15.2 & 16.0 & 15.2 & 16.9 & 14.9 & 16.5 & 16.6 & 17.9 & 18.9 & 21.4 & 21.6 & 14.7 & 16.8 & 16.6 & 18.2 & 16.7 & 17.8 & 16.0 & 20.1 & 18.5 & 17.3 (\textcolor{MidnightBlue}{-27.3\%})\\
&EB-Net$^\dag$~\cite{chen2023more}        & 28.0 & 29.8 & 27.4 & 31.2 & 26.5 & 30.3  & 30.5  & 32.1 & 33.2 & 35.8 & 36.3 & 27.3 & 30.3 & 27.0 & 30.6 & 30.6 & 30.7 & 33.7 & 35.6& 30.1 & 30.9 (\textcolor{MidnightBlue}{-22.4\%})\\ 
&\cc\textbf{HiKER-SGG} & \cc\textbf{31.1} & \cc\textbf{33.3} & \cc\textbf{31.5} & \cc\textbf{35.4} & \cc\textbf{28.5}  & \cc\textbf{35.0}  & \cc\textbf{34.1}  & \cc\textbf{36.5} & \cc\textbf{37.7} & \cc\textbf{39.8} & \cc\textbf{40.8} & \cc\textbf{30.5} & \cc\textbf{33.7} & \cc\textbf{31.3} & \cc\textbf{34.2} & \cc\textbf{33.5} & \cc\textbf{34.9} & \cc\textbf{37.1} & \cc\textbf{39.8} & \cc\textbf{32.6} & \cc\textbf{34.6} (\textcolor{MidnightBlue}{\cc\textbf{-17.8\%}})\\
\cmidrule{2-23}
&GB-Net$^\dag$~\cite{zareian2020bridging} & 10.3 & 10.6 & 10.4 & 11.6 & 10.4 & 10.9 & 10.7 & 11.9 & 12.3 & 13.7 & 13.8 & 10.0 & 11.1 & 10.8 & 11.7 & 11.1 & 11.2 & 10.5 & 13.0 & 12.1 & 11.4 (\textcolor{MidnightBlue}{-25.5\%})\\
&EB-Net$^\dag$~\cite{chen2023more}        & 21.7 & 22.8 & 20.4 & 24.9 & 19.6 & 23.2 & 23.8 & 23.2 & 24.6 & 27.5 & 28.0 & 20.1 & 23.1 & 21.1 & 23.6 & 24.0 & 23.4 & 25.6 & 27.3 & 22.9 & 23.5 (\textcolor{MidnightBlue}{-23.7\%})\\
&\cc\textbf{HiKER-SGG} & \cc\textbf{24.8} & \cc\textbf{25.8} & \cc\textbf{24.8} & \cc\textbf{27.5} & \cc\textbf{22.4} & \cc\textbf{27.4} & \cc\textbf{26.4} & \cc\textbf{27.8} & \cc\textbf{28.7} & \cc\textbf{31.1} & \cc\textbf{31.5} & \cc\textbf{23.3} & \cc\textbf{26.0} & \cc\textbf{24.3} & \cc\textbf{26.5} & \cc\textbf{26.3} & \cc\textbf{26.8} & \cc\textbf{28.5} & \cc\textbf{30.9} & \cc\textbf{24.9} & \cc\textbf{26.8} (\textcolor{MidnightBlue}{\cc\textbf{-19.8\%}})\\
\midrule
\multirow{6}{*}[-0.9ex]{\centering \rotatebox{90}{mR@50: C/UC}}&GB-Net$^\dag$~\cite{zareian2020bridging} & 27.5 & 28.7 & 27.6 & 30.8 & 26.4 & 29.8 & 29.9 & 31.9 & 33.8 & 37.2 & 37.6 & 26.3 & 29.9 & 30.0 & 33.0 & 29.5 & 32.3 & 28.7 & 35.8 & 32.8 & 31.0 (\textcolor{MidnightBlue}{-24.6\%})\\
&EB-Net$^\dag$~\cite{chen2023more}        & 42.1 & 43.7 & 41.5 & 44.9 & 40.2 & 45.6 & 44.2 & 46.9 & 47.7 & 50.4 & 51.2 & 41.2 & 44.1 & 41.4 & 45.1 & 45.4 & 45.5 & 48.4 & 49.7 & 44.6 & 45.2 
 (\textcolor{MidnightBlue}{-17.7\%})\\ 
&\cc\textbf{HiKER-SGG} & \cc\textbf{46.7} & \cc\textbf{48.4} & \cc\textbf{46.9} & \cc\textbf{50.2} & \cc\textbf{43.2} & \cc\textbf{49.6} & \cc\textbf{48.3} & \cc\textbf{51.3} & \cc\textbf{52.5} & \cc\textbf{55.1} & \cc\textbf{55.9} & \cc\textbf{45.0} & \cc\textbf{48.1} & \cc\textbf{46.0} & \cc\textbf{49.9} & \cc\textbf{48.6} & \cc\textbf{50.0} & \cc\textbf{52.4} & \cc\textbf{54.8} & \cc\textbf{47.0} & \cc\textbf{49.5} 
 (\textcolor{MidnightBlue}{\cc\textbf{-14.5\%}})\\
\cmidrule{2-23}
&GB-Net$^\dag$~\cite{zareian2020bridging} & 13.3 & 13.6 & 13.3 & 15.1 & 13.6 & 14.1 & 14.0 & 15.4 & 15.6 & 17.4 & 17.5 & 13.0 & 14.5 & 14.4 & 15.2 & 14.5 & 14.6 & 13.6 & 16.6 & 15.4 & 14.7 
 (\textcolor{MidnightBlue}{-24.2\%})\\
&EB-Net$^\dag$~\cite{chen2023more}        & 24.8 & 27.6 & 25.6 & 28.3 & 25.9 & 28.9 & 29.4 & 29.3 & 30.5 & 32.0 & 32.8 & 26.1 & 28.6 & 26.3 & 27.9 & 29.2 & 28.6 & 30.8 & 31.8 & 27.2 & 28.6 
(\textcolor{MidnightBlue}{-22.1\%})\\ 
&\cc\textbf{HiKER-SGG} & \cc\textbf{30.1} & \cc\textbf{31.7} & \cc\textbf{30.4} & \cc\textbf{33.2} & \cc\textbf{28.3} & \cc\textbf{33.3} & \cc\textbf{32.1} & \cc\textbf{34.1} & \cc\textbf{34.4} & \cc\textbf{37.3} & \cc\textbf{37.4} & \cc\textbf{28.8} & \cc\textbf{31.7} & \cc\textbf{30.1} & \cc\textbf{32.9} & \cc\textbf{32.5} & \cc\textbf{32.2} & \cc\textbf{34.5} & \cc\textbf{36.7} & \cc\textbf{30.4} & \cc\textbf{32.6} 
 (\textcolor{MidnightBlue}{\cc\textbf{-17.0\%}})\\
\midrule
\multirow{6}{*}[-0.3ex]{\centering \rotatebox{90}{mR@100: C/UC}}&GB-Net$^\dag$~\cite{zareian2020bridging} & 40.1 & 41.9 & 40.1 & 43.8 & 37.8 & 42.9 & 42.7 & 45.1 & 47.1 & 50.8 & 51.7 & 37.8 & 42.8 & 42.9 & 46.6 & 42.5 & 46.1 & 41.2 & 49.6 & 45.9 & 44.0 
 (\textcolor{MidnightBlue}{-20.6\%})\\
&EB-Net$^\dag$~\cite{chen2023more}        & 54.7 & 56.0 & 52.9 & 56.8 & 52.4 & 55.6 & 55.3 & 58.4 & 59.9 & 61.6 & 61.1 & 53.3 & 55.0 & 54.3 & 57.7 & 56.4 & 57.6 & 59.0 & 60.7 & 54.8 & 56.7 
 (\textcolor{MidnightBlue}{-14.5\%})\\
&\cc\textbf{HiKER-SGG} & \cc\textbf{59.3} & \cc\textbf{60.3} & \cc\textbf{58.6} & \cc\textbf{62.3} & \cc\textbf{55.6} & \cc\textbf{61.9} & \cc\textbf{59.8} & \cc\textbf{63.4} & \cc\textbf{64.0} & \cc\textbf{66.9} & \cc\textbf{67.4} & \cc\textbf{56.4} & \cc\textbf{60.1} & \cc\textbf{58.4} & \cc\textbf{62.3} & \cc\textbf{59.8} & \cc\textbf{62.1} & \cc\textbf{63.7} & \cc\textbf{66.3} & \cc\textbf{58.9} & \cc\textbf{61.4} 
 (\textcolor{MidnightBlue}{\cc\textbf{-11.3\%}})\\
\cmidrule{2-23}
&GB-Net$^\dag$~\cite{zareian2020bridging} & 14.8 & 15.1 & 14.6 & 16.6 & 15.1 & 15.6 & 15.6 & 16.9 & 17.1 & 19.1 & 19.0 & 14.4 & 16.0 & 16.0 & 16.8 & 16.1 & 16.1 & 15.0 & 18.1 & 17.0 & 16.3 
(\textcolor{MidnightBlue}{-22.0\%})\\
&EB-Net$^\dag$~\cite{chen2023more}        & 28.7 & 30.1 & 27.8 & 31.9 & 27.1 & 31.1 & 30.5 & 32.8 & 32.4 & 36.1 & 35.7 & 28.2 & 30.9 & 28.4 & 30.9 & 31.4 & 31.0 & 31.8 & 33.9 & 29.6 & 31.0 
(\textcolor{MidnightBlue}{-20.9\%})\\
&\cc\textbf{HiKER-SGG} & \cc\textbf{32.7} & \cc\textbf{33.8} & \cc\textbf{32.6} & \cc\textbf{36.0} & \cc\textbf{30.4} & \cc\textbf{35.7} & \cc\textbf{34.7} & \cc\textbf{36.3} & \cc\textbf{36.7} & \cc\textbf{39.9} & \cc\textbf{39.7} & \cc\textbf{31.1} & \cc\textbf{34.2} & \cc\textbf{32.7} & \cc\textbf{35.4} & \cc\textbf{34.9} & \cc\textbf{35.4} & \cc\textbf{37.1} & \cc\textbf{39.2} & \cc\textbf{32.6} & \cc\textbf{35.1} 
 (\textcolor{MidnightBlue}{\cc\textbf{-14.8\%}})\\
\bottomrule
\end{tabular}
}
\vspace{-20pt}
\end{center}
\end{table*}
